Gender Effect on Face Recognition for a Large Longitudinal Database

Aging or gender variation can affect the face recognition performance dramatically. While most of the face recognition studies are focused on the variation of pose, illumination and expression, it is important to consider the influence of gender effect and how to design an effective matching framework. In this paper, we address these problems on a very large longitudinal database MORPH-II which contains 55,134 face images of 13,617 individuals. First, we consider four comprehensive experiments with different combination of gender distribution and subset size, including: 1) equal gender distribution; 2) a large highly unbalanced gender distribution; 3) consider different gender combinations, such as male only, female only, or mixed gender; and 4) the effect of subset size in terms of number of individuals. Second, we consider eight nearest neighbor distance metrics and also Support Vector Machine (SVM) for classifiers and test the effect of different classifiers. Last, we consider different fusion techniques for an effective matching framework to improve the recognition performance.

==> referencest.tex <==
@article{towns2014xsede,
  title={XSEDE: accelerating scientific discovery},
  author={Towns, John and Cockerill, Timothy and Dahan, Maytal and Foster, Ian and Gaither, Kelly and Grimshaw, Andrew and Hazlewood, Victor and Lathrop, Scott and Lifka, Dave and Peterson, Gregory D and others},
  journal={Computing in Science \& Engineering},
  volume={16},
  number={5},
  pages={62--74},
  year={2014},
  publisher={IEEE}
}

@article{li2011discriminative,
  title={A discriminative model for age invariant face recognition},
  author={Li, Zhifeng and Park, Unsang and Jain, Anil K},
  journal={IEEE transactions on information forensics and security},
  volume={6},
  number={3},
  pages={1028--1037},
  year={2011},
  publisher={IEEE}
}

@article{kevin2017,
  title={Do I Know You? Optimizing the Facial Recognition System Through Distance Metrics},
  author={Park, Kevin},
  journal={UNCW NSF REU Summer 2017},
  year={2018},
}

@article{morgan2017,
  title={Face Recognition Optimization on the Morph-II Database},
  author={Ferguson, Morgan},
  journal={UNCW NSF REU Summer 2017},
  year={2018},
}


@article{best2018longitudinal,
  title={Longitudinal study of automatic face recognition},
  author={Best-Rowden, Lacey and Jain, Anil K},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={40},
  number={1},
  pages={148--162},
  year={2018},
  publisher={IEEE}
}

@article{polikar2006ensemble,
  title={Ensemble based systems in decision making},
  author={Polikar, Robi},
  journal={IEEE Circuits and systems magazine},
  volume={6},
  number={3},
  pages={21--45},
  year={2006},
  publisher={IEEE}
}

@article{liu2009comparative,
  title={A COMPARATIVE STUDY OF DISTANCE METRICS USED IN FACE RECOGNITION.},
  author={Liu, Zunxiong and Xu, Zheng and Hu, Linfeng},
  journal={Journal of Theoretical \& Applied Information Technology},
  volume={5},
  number={2},
  year={2009}
}

@inproceedings{turk1991face,
  title={Face recognition using eigenfaces},
  author={Turk, Matthew A and Pentland, Alex P},
  booktitle={Computer Vision and Pattern Recognition, 1991. Proceedings CVPR'91., IEEE Computer Society Conference on},
  pages={586--591},
  year={1991},
  organization={IEEE}
}

@article{welling2005fisher,
  title={Fisher linear discriminant analysis},
  author={Welling, Max},
  journal={Department of Computer Science, University of Toronto},
  volume={3},
  number={1},
  year={2005}
}

@incollection{yambor2002analyzing,
  title={Analyzing PCA-based face recognition algorithms: Eigenvector selection and distance measures},
  author={Yambor, Wendy S and Draper, Bruce A and Beveridge, J Ross},
  booktitle={Empirical evaluation methods in computer vision},
  pages={39--60},
  year={2002},
  publisher={World Scientific}
}

@article{delac2005independent,
  title={Independent comparative study of PCA, ICA, and LDA on the FERET data set},
  author={Delac, Kresimir and Grgic, Mislav and Grgic, Sonja},
  journal={International Journal of Imaging Systems and Technology},
  volume={15},
  number={5},
  pages={252--260},
  year={2005},
  publisher={Wiley Online Library}
}

@article{melivsek2008support,
  title={Support vector machines, PCA and LDA in face recognition},
  author={Meli{\v{s}}ek, J{\'a}n Mazanec—Martin and Pavlovicov{\'a}, Milo{\v{s}} Oravec—Jarmila},
  journal={J. Electr. Eng},
  volume={59},
  pages={203--209},
  year={2008}
}

@inproceedings{lu2003combining,
  title={Combining classifiers for face recognition},
  author={Lu, Xiaoguang and Wang, Yunhong and Jain, Anil K},
  booktitle={Multimedia and Expo, 2003. ICME'03. Proceedings. 2003 International Conference on},
  volume={3},
  pages={III--13},
  year={2003},
  organization={IEEE}
}

@inproceedings{phillips1999support,
  title={Support vector machines applied to face recognition},
  author={Phillips, P Jonathon},
  booktitle={Advances in Neural Information Processing Systems},
  pages={803--809},
  year={1999}
}

@incollection{zhao1998discriminant,
  title={Discriminant analysis of principal components for face recognition},
  author={Zhao, Wenyi and Krishnaswamy, Arvindh and Chellappa, Rama and Swets, Daniel L and Weng, John},
  booktitle={Face Recognition},
  pages={73--85},
  year={1998},
  publisher={Springer}
}

@article{toygar2003face,
  title={Face recognition using PCA, LDA and ICA approaches on colored images},
  author={Toygar, {\"O}nsen and Adnan, Acan},
  journal={IU-Journal of Electrical \& Electronics Engineering},
  volume={3},
  number={1},
  pages={735--743},
  year={2003}
}

@inproceedings{marcialis2002fusion,
  title={Fusion of LDA and PCA for Face Verification},
  author={Marcialis, Gian Luca and Roli, Fabio},
  booktitle={International Workshop on Biometric Authentication},
  pages={30--37},
  year={2002},
  organization={Springer}
}

@article{satonkarface,
  title={FACE RECOGNITION USING DIFFERENT DISTANCE MEASURES TECHNIQUES},
  author={Satonkar, Suhas S and Kurhe, Ajay B and Khanale, Prakash B}
}
